Accelerated K-Serial Stable Coalition for Dynamic Capture and Resource Defense

Coalition is an important mean of multi-robot systems to collaborate on common tasks. An adaptive coalition strategy is essential for the online performance in dynamic and unknown environments. In this work, the problem of territory defense by large-scale heterogeneous robotic teams is considered. The tasks include exploration, capture of dynamic targets, and perimeter defense over valuable resources. Since each robot can choose among many tasks, it remains a challenging problem to coordinate jointly these robots such that the overall utility is maximized. This work proposes a generic coalition strategy called K-serial stable coalition algorithm. Different from centralized approaches, it is distributed and complete, meaning that only local communication is required and a K-serial Stable solution is ensured. Furthermore, to accelerate adaptation to dynamic targets and resource distribution that are only perceived online, a heterogeneous graph attention network based heuristic is learned to select more appropriate parameters and promising initial solutions during local optimization. Compared with manual heuristics or end-to-end predictors, it is shown to both improve online adaptability and retain the quality guarantee. The proposed methods are validated via large-scale simulations with 170 robots and hardware experiments of 13 robots, against several strong baselines such as GreedyNE and FastMaxSum.

==> contents/alg.tex <==
%==============================
\subsubsection{Algorithm-improvment}\label{subsubsec:alg-improve}

Consider the simple formulation~$(\mathcal{A},\,\Omega,\, f,\,\mathcal{K})$,
where~$\mathcal{A}=\{a_1, \cdots, a_N\}$ is the set of agents,
$\Omega=\{\omega_1,\cdots, \omega_M\}$ is the set of tasks,
$f:2^A \times \Omega \rightarrow R^+$ is the utility function, $\mathcal{K}=\{k1,k2,\cdots,k_N\}$ is the set of depth limit of search tree for all agents, which provides a way for us to selectively increase or decrease  the depth of search tree for agents in different areas of the map.

We denote coalition structure $\mathcal{S} = \{\mathcal{C}_1, \cdots \mathcal{C}_M\}$ with each $\mathcal{C}_j$ being responsible for a specific task $\omega_j$,
and each agent $a_i$ can attend at most one task simultaneously， namely $\mathcal{C}_i\cap\mathcal{C}_j=\emptyset,\forall i\neq j$.
In the following description, $\nu$ is used to denote an assignment and has following format:
$$
    \nu = ((\omega_j,a_i \in \mathcal{C}_j, u_j=f(\mathcal{C}_j,\omega_j))
    ,\ \forall j \in \{1,2,\cdots,M\})
$$  

%  where $\mathcal{A}_j$ is a subset of set $\mathcal{A}$.
  
 
 We denote the utility of assignment $\nu$ as $U(\nu)$, which is simply defined as the mean value of all coalitions' utility in $\nu$.
 $$U(\nu)=mean_{\mathcal{C}_j \in \mathcal{S}}\{u_j\}$$



Distributed search tree construction is the core of our algorithm. Each search tree $\mathcal{T}_i(\nu_0)$ has a depth limit $k_i$ and is locally formed by consecutive switch operations from an root node $\nu_0$ created by agent i. Each node of the search tree is an assignment. Considering that what we want to achieve is a distributed search, it is not suitable to build a complete search tree on each agent, because it means that the agent must has the global information. Therefore we take an approach where only the extended form of leaf nodes are passed between agents as follow:
$$\pi=(\nu_0,\nu_d,\mathcal{H},k,d)\ ,\ \mathcal{H}=\{\ h_i=(\Hat{a}_i,\Hat{\omega}_i,\Hat{\omega}_i^+)\ |\ i \in \{1,2,\cdots ,d\}\ \}$$

$\pi$ is an extended form of the leaf node $\nu_d$. As defined above, in addition to node $\nu_d$, $\pi$ also contains the root node $\nu_0$, the switch transformation history $\mathcal{H}$, the depth limit k and the current depth d.  $h_i=(\Hat{a}_i,\hat{\omega}_i,\hat{\omega}_i^+) \in \mathcal{H}$ represents that the i-th switch was conducted by agent $\Hat{a}_i$ and it switched from task $\Hat{\omega}_i$ to $\Hat{\omega}_i^+$ . 

Each agent has a finite memory $\mathcal{M}$:
 $$\mathcal{M}=(\Pi_i,\nu_i^*,\rho_i^*)$$
 
 where $\Pi_i$ is the node set, $\nu_i^*,\rho_i^*$ are the best assignment and the corresponding maximum utility.

In the following, We define a special map $\mathcal{L}$ that maps the two assignment $\nu_1\ and\ \nu_2$ to the set of all targets involved in switch transformation from $\nu_1$ to $\nu_2$.
$$\mathcal{L}(\nu_1,\nu_2)=\{\hat{\omega}_1,\cdots,\hat{\omega}_n\}$$


 After the basic definition, a brief description of the overall idea of our algorithm can be given. Initially, each agent creates an initial root node and sets the depth limit of the search tree according to the given parameters $\mathcal{K}$. The agent realizes the distributed construction of the search tree by receiving leaf nodes, generating new leaf nodes, and sending them to neighbors. A leaf node will stop propagating when it has reached the depth limit or has become a child node. In the process of distributed search, once an agent finds a leaf node $\nu*$ with higher utility, it will replace the root node $\nu_{0}$ with $\nu*$ for all leaf nodes stored in $\Pi_i$. 
 
 Here we need to add a new definition using map $\mathcal{L}$ defined before. We define an replacement to be conflicting if and only if the new root node $\nu^*$ and the extended leaf node $\pi=(\nu_0,\nu_d,H,K,d)\in \Pi_i$ satisfies: $$\mathcal{L}(\nu_0,\nu_0^+)\cap\mathcal{L}(\nu_0,\nu_d)\neq\emptyset$$
 
 If the replacement is not conflicting, the agent will directly recalculate the utility of the corresponding leaf node in $\Pi_i$, otherwise the parent node of the leaf node will be continuously traced back until the conflict is eliminated, and a partial search tree reconstruction will be performed from the conflict-free node. Finally, all agents will reach a consensus on the optimal root node. When the algorithm converges, the root node can prove to be a $\mathcal{K}$-serial Nash-stable solution.
 

Each agent~$a_i\in \mathcal{A}$ performs asynchronously the following procedure:
\begin{enumerate}
\item At $t=0$:
  \begin{enumerate}
  \item Check the set of visible tasks~$\Omega_i=\{\omega_1, \omega_2,\cdots, \omega_J\} \subseteq \Omega$.
  \item Compute the initial assignment $\nu$
    $$
    \nu = ((\omega_{nearest}, a_i, f(\{a_i\}, \omega_{j})),
    (\omega_{j'}, \emptyset, \infty),\forall j'\neq j )
    $$
    Where $\omega_{nearest}$ is the nearest target to agent $a_i$.\\
    Create the root node of K-tree:
    $$\pi_{root}= (\nu,\nu,\emptyset,k_i,0)$$
    % Where $K_n$ is the upper bound of the distance between root and leaf. In other words, $K_n$ is the maximum height of the search tree started from agent $a_i$. d is the distance between current leaf node and root node with initial value 0.
  \item  Initialize memory $\mathcal{M}$:
  $$\Pi_i=\emptyset,\ \nu_i^*=\nu,\ \rho_i^*=U(\nu)$$
  \item  Send the following message to itself:
  $$
  \boldsymbol{\mu}_{i\rightarrow i} = (\rho_0,\rho_d, \pi_{root}),
  $$
  where~$\rho_0=U(\nu),\rho_d=U(\nu)$.
  
  \end{enumerate}
\item For \emph{each} $\pi\in \Pi_i,\ \pi= (\nu_0,\nu_d,\mathcal{H},k,d),\ \mathcal{H}=\{\ h_i=(\Hat{a}_i,\Hat{\omega}_i,\Hat{\omega}_i^+)\ |\ i \in \{1,2,\cdots ,d\}\ \}$:

If $d<k$ and $\Hat{\omega}_i\neq\Hat{\omega}_i^+$, send a message $\boldsymbol{\mu}_{i\rightarrow j}$ to all neighbors~$j\in \mathcal{N}_{\Hat{\omega}_d} \cup \mathcal{N}_{\Hat{\omega}_d^+}$:
  $$
  \boldsymbol{\mu}_{i\rightarrow j} = (\rho_0,\rho_d, \pi),
  $$
  where~$\rho_0=U(\nu_0),\rho_d=U(\nu_d)$. 
  
  Remove the node $\pi$ that have been sent to neighbors from $\Pi_i$. 


\item Receive message~$\boldsymbol{\mu}_{j\rightarrow i}$ ,  and remove the duplicate message. Set flag $\boldsymbol{f}=False$ to denote whether the best assignment update occurs in the message-receiving process.
  Then for each received message~$\boldsymbol{\mu}_{j\rightarrow i}=(\rho_0,\rho_d, \pi), \pi=(\nu_0,\nu_d,\mathcal{H},k,d)$:
  \begin{enumerate}
  \item if $\rho_0>\rho_i^*$, update best assignment: $\nu_i^{*}=\nu_0$, $\rho_i^{*}=U(\nu_0)$, and set flag $\boldsymbol{f}=True$.

  
  \item 
    \begin{enumerate}
        \item If $|\mathcal{H}|=d$:
        Check all known tasks in~$\nu_d =     ((\omega_j,\mathcal{A}_j, u_j)
        ,\ \forall j \in \{1,2,\cdots,M\})$.
        For \emph{each} task~$\omega \in \nu_d$ that is     known to agent~$i$,
        generate new assignment~$\nu_d^+$
        by assign~$i$ to~$\omega$.
        $$\pi^+=(\nu_0,\nu^+_{d},\mathcal{H}\cup\{(\Hat    {a}_{d+1},\omega_s,\omega)\},k_i,d+1)$$
    
    where s satisfies $i\in \mathcal{A}_s$.
    
        \item if $|\mathcal{H}|>d$:
        Reconstruct conflicting part of the search tree from this node. The next switch operation has been preset in $\mathcal{H}$ in advance as $h_{d+1}=(\Hat{a}_{d+1},\Hat{\omega}_{d+    1},\Hat{\omega}_{d+1}^+)$. So we generate a new assignment $\nu_d^+$ by assign i to $\Hat{\omega}_{d+1}^+$, and the extended form is also generated as follow:
        $$\pi^+=(\nu_0,\nu^+_{d},\mathcal{H},k_i,d+1)$$
    \end{enumerate}
    
  \item If $\rho_d^+=U(\nu_d^+)>\rho_{i}^*$, update best assignment: $\nu_i^{*}=\nu_d^+$,$\rho_i^{*}=U(\nu_d^+)$, and set flag $\boldsymbol{f}=True$.
  
  \item For each $\pi^+=(\nu_0,\nu_d,\mathcal{H},k,d)$ generated in (b), if $d$ is less than $k$, save~$\pi^+$ to~$\Pi_i$. Otherwise, do nothing to $\Pi_i$.
  \end{enumerate}
\item If flag $\boldsymbol{f}$ is True, do the root node replacement.
For each $\pi$ in $\Pi_i$:
$$\pi=(\nu_0,\nu_d,\mathcal{H},k,d)\ \ \mathcal{H}=\{\ h_i=(a_i,\Hat{\omega}_i,\Hat{\omega}_i^+)\ |\ i \in \{1,2,\cdots ,d\}\ \}$$
    \begin{enumerate}
    \item if $\mathcal{L}(\nu_0,\nu_i^*)\cap\mathcal{L}(\nu_0,\nu_d)=\emptyset$: 
    
    Simply combine the change $\nu_0\rightarrow\nu_i^*$ and $\nu_0\rightarrow\nu_d$ and then we can get the new leaf node $\nu_d^+$. Replace $\pi$ in $\Pi_i$ with $\pi^+=(\nu_i^*,\nu_d^+,\mathcal{H},k,d)$. Since the replacement is not conflicting, we can calculate the utility of new assignment $\rho_d^+$ by simply add the utility change from $\nu_0$ to $\nu_i^*$:
    $$\rho_d^+=\rho_d+\rho_i^*-\rho_0$$
    
    If $\rho_d^+>\rho_i^*$, update best assignment: $\nu_i^{*}=\nu_d^+$, $\rho_i^{*}=\rho_d^+$, and then back to the start of Step (4).
    \item If $\mathcal{L}(\nu_0,\nu_i^*)\cap\mathcal{L}(\nu_0,\nu_d)\neq\emptyset$:
    
    According to the switch history $\mathcal{H}$, we can restore all child nodes $ \nu_1,\cdots,\nu_{d-1}$ in the switch chain based on the root node $\nu_0$. 
    Calculate the max index j that satisfies $\mathcal{L}(\nu_0,\nu_i^*)\cap\mathcal{L}(\nu_0,\nu_j)=\emptyset$. Then create a new node $\pi^+=(\nu_i^*,\nu_j,\{h_1,h_2,\cdots,h_j,h_{j+1}\},k,j)$, and send a message $\boldsymbol{\mu}_{i\rightarrow \Hat{a}_{j+1}}$ to agent $\Hat{a}_{j+1}$:
    $$
    \boldsymbol{\mu}_{i\rightarrow \Hat{a}_{j+1}} = (\rho_0,\rho_d, \pi^+),
    $$
  where~$\rho_0=U(\nu_i^*),\rho_d=U(\nu_j)$.
  
  Remove $\pi$ from $\Pi_i$.
    \end{enumerate}  
\item Back to Step (2)
\end{enumerate}


% \textcolor{red}{
%   1. Add the remark/example that the utility function is not additive.
%    Should $\nu$ be a set or a sequence?
% 2. Is $\mathcal{K}$ required to be consecutive or any integer in $[1,N]$ or upper/lower bound?
% 3. the definition of $Mean$ can be more explicit, right?
% 4. "distributed search tree construction" ---> "the distributed construction of search trees"
% 5. The tree $\mathcal{T}_i$ should be defined more formally.
% 6. The under-scripts are a bit sloopy, i.e., $i$ is used both for indexing agent and tasks.
%   Try maybe $m$ for $M$, $n$ for $N$, and $i,j$ for $I,J$.
% 7. I would recommend to replace "extended leaf nodes" with a "message",
%   and explicitly describe it as a part of the communication process.
% 8. I think the "switch operation" should be formally defined before introducing the message.
%   And it would be part of the definition of the search tree, as the branching method.
% 9. the depth limit $k$ of whom?
% 10. what is the current depth?
% 11. I feel that the message~$\pi$ can be more streamlined as a ``path" from $\nu_0$ to $\nu_d$.
%   It would include the most information, and cleaner, less ad-hock.
% 12. $\mathcal{M}$ should be indexed.
% 13. What is the purpose of~$\Pi_i$? I think agent~$i$ would need to store its entire tree anyway?
% 14. $L$  should be defined formally, using~$\nu$.
% 15. Must $\mathcal{K}$ be given? can it be adjusted in a distributed way?
%   i.e., each agent starts from $k=1$, and increase it incrementally after convergence.
% 16. The description of sending "leaf nodes" is not clear. I would recommend to use messages.
%   See comment above.
% 17. "or has become a child node". Isn't a leaf node always a child node?
% 18. The description is hard to follow before the actual algorithm is given.
% 19. Alg.1.b should the root of a tree be $\nu$? $\pi$ is the message format, right?
% 20. Alg.1.c the total utility is hard to compute locally. Needs improvement.
% 21. Alg.2 why $\check{\omega}_i \neq \check{\omega}^+_i$?
% 22. Alg.3 the discussion involving $\nu$ and $\pi$ is a bit confusing.
% 23. Alg.3.b.ii what is "preset"?  what is $i$?
% 24. Alg.4.a how is the new leaf node $\nu^+_d$ defined?
% 25. I actually do not get why the replacement is needed. To discuss.
% 26. Alg.4.b related to the previous comment,
%     a (augmented) path would include the sequence of nodes already.
% 27. Alg.4.b is $\nu_j$ ensured to be found?
% }





==> contents/limitation.tex <==

\section{Current Limitations}\label{sec:limitation}



%==============================
\subsection{Generalization from Very Few Demos}\label{subsec:limit-few}


%==============================
\subsection{Multiple Branches for One Skill}\label{subsec:limit-branch}

%==============================
\subsection{Manual Conditioning in Task Graph}\label{subsec:manual-specification}


==> contents/preliminary.tex <==
\section{Preliminaries}\label{sec:preliminary}

% ==========
\subsection{Apollonius Circle}\label{subsec:circle}
Consider two points~$p_1,\,p_2\in \mathbb{R}^2$ and a given ratio~$\alpha>0$.
As shown in Fig.~\ref{fig:appolonius}, the notion of Apollonius Circle is introduced in~\cite{moll2018pursuit},
defined as the set of points:
\begin{equation}\label{eq:circle}
  \mathcal{C}(p_1,p_2,\alpha)=\{p\in \mathbb{R}^2\,|\,\|p-p_1\| \leq \alpha \|p-p_2\|\},
\end{equation}
where~$\alpha>0$ is a given parameter.
This circle is particularly relevant to pursuer-evader games.
Namely,
if agent~$1,2$ start from~$p_1,\,p_2$ and a velocity ratio~$\alpha$,
then agent~$1$ can reach any point within~$\mathcal{C}$
earlier than agent~$2$,
i.e., agent~$1$ can capture agent~$2$ at any point within~$\mathcal{C}$.
Such notion can also be extended to the scenario of multiple pursuers,
by computing the intersection of different Apollonius Circles.
More detailed analyses can be found in~\cite{moll2018pursuit}.
\todo{check $\geq$ and ``intersection''.}
\begin{figure}
  \centering
  \includegraphics[width=0.5\linewidth]{figures/Apollonius.jpg}
  \caption{Illustration of Apollonius Circle.
  \todo{Replace with two or three plots to illustrate the overlapping of AC.}
  }
  \label{fig:appolonius}
\end{figure}
% ==========
\subsection{Coalition Formation}\label{subsec:coalition}
The general problem of coalition formation for multi-agent systems is defined in~\cite{rahwan2015coalition,li2020anytime}
by the 3-tuple~$(\mathcal{A},\,\mathcal{T},\,f)$, where~$\mathcal{A}$ is the set of agents,
$\mathcal{T}$ is a set of tasks,
and $f: 2^\mathcal{A}\times\mathcal{T} \rightarrow \mathbb{R}_{>0}$ is the utility function.
A coalition formed by a subset of agents~$\mathcal{A}_j\subset \mathcal{A}$ performing task~$\tau_j\in \mathcal{T}$
yields the utility~$f(\mathcal{A}_j,\,\tau_j)$.
Furthermore, a coalition structure formed by the set of coalitions~$\mathcal{A}_1,\cdots,\mathcal{A}_J$
is valid for a given set of tasks~$\{\tau_1,\cdots,\tau_J\}$
if~$\mathcal{A}_j\subset \mathcal{A}$ and~$\mathcal{A}_{j_1}\cap \mathcal{A}_{j_2} = \emptyset$,
$\forall j,j_1,j_2\in\{1,\cdots,J\}$,
i.e., each agent can belong to the coalition of at most one task.
Thus, the total utility is given by~$\sum_j f(\mathcal{A}_j,\,\tau_j)$, commonly used as the
objective to maximize for choosing the coalition structure.
As stated in~\cite{rahwan2015coalition}, the coalition formation problem is a combinatorial optimziation
problem of which the worst-case complexity for computing the global optimal solution
is exponential to the number of agent and the number of tasks.
Thus, an important notion of local optimality is introduced as the \emph{Nash Equilibrium}, i.e.,
a coalition structure is a Nash Equilibrium~\cite{halpern2008beyond} if no single agent
can improve the total utility by changing its own coalition.


==> contents/related.tex <==
% ==============================
\section{Related Work}\label{sec:related}

%%%%%%%%%%%
\subsection{Coalition Structure Generation}\label{related:coaliation}

\todo{I think it makes more sense to first introduce other task assignment algorithms,
  and emphasize the limitation that most work relies on fixed agent-to-task cost/gain.
  This would then motivate CSG, where the utility is defined for a coalition.
This should be a very important point to emphasize.}



%%%%%%%%%%%
\subsection{Pursuit-Evasion Problems}\label{related:pursuit}
\todo{This part is unnecessarily long, and we should add related work for the other two tasks,
e.g., exploration and encirclement.}


% Though being an active research field on its own,
% the problem of dynamic tracking of moving targets,
% see~\cite{liu2020rumor,dames2017detecting}, has not been analyzed together
% with the capture problem.

